Library Event Matching event classification algorithm for electron neutrino interactions in the NOvA detectors

We describe the Library Event Matching classification algorithm implemented for use in the NOvA $\nu_\mu \rightarrow \nu_e$ oscillation measurement. Library Event Matching, developed in a different form by the earlier MINOS experiment, is a powerful approach in which input trial events are compared to a large library of simulated events to find those that best match the input event. A key feature of the algorithm is that the comparisons are based on all the information available in the event, as opposed to higher-level derived quantities. The final event classifier is formed by examining the details of the best-matched library events. We discuss the concept, definition, optimization, and broader applications of the algorithm as implemented here. Library Event Matching is well-suited to the monolithic, segmented detectors of NOvA and thus provides a powerful technique for event discrimination.

==> Makefile <==
all: color bw

color:
	latex lem.tex
	latex lem.tex
	dvips lem.dvi -o lem_color.ps
	ps2pdf -dPDFSETTINGS=/prepress -dSubsetFonts=true -dEmbedAllFonts=true -dMaxSubsetPct=100 -dCompatibilityLevel=1.3 lem_color.ps

bw:
	latex "\def\BW{}\input{lem}"
	latex "\def\BW{}\input{lem}"
	dvips lem.dvi -o lem_bw.ps
	ps2pdf -dPDFSETTINGS=/prepress -dSubsetFonts=true -dEmbedAllFonts=true -dMaxSubsetPct=100 -dCompatibilityLevel=1.3 lem_bw.ps

